Optimizing Reported Age of Information with Short Error Correction and Detection Codes

Timely sampling and fresh information delivery are important in 6G communications. This is achieved by encoding samples into short packets/codewords for transmission, with potential decoding errors. We consider a broadcasting base station (BS) that samples information from multiple sources and transmits to respective destinations/users, using short-blocklength cyclic and deep learning (DL) based codes for error correction, and cyclic-redundancy-check (CRC) codes for error detection. We use a metric called reported age of information (AoI), abbreviated as RAoI, to measure the freshness of information, which increases from an initial value if the CRC reports a failure, else is reset. We minimize long-term average expected RAoI, subject to constraints on transmission power and distortion, for which we obtain age-agnostic randomized and age-aware drift-plus-penalty policies that decide which user to transmit to, with what message-word length and transmit power, and derive bounds on their performance. Simulations show that longer CRC codes lead to higher RAoI, but the RAoI achieved is closer to the true, genie-aided AoI. DL-based codes achieve lower RAoI. Finally, we conclude that prior AoI optimization literature with finite blocklengths substantially underestimates AoI because they assume that all errors can be detected perfectly without using CRC.

==> Introduction.tex <==
Due to the increasing demand for real-time updates in various emerging applications,   such as video surveillance and autonomous driving, design and optimization of wireless networks for delivering information freshly has gained great research interest recently. 
A metric called age of information (AoI), defined as the time elapsed since the generation of the last successfully received update packet at the destination about its source, as a measure of timeliness of information was  proposed in \cite{age_first} and has been widely studied \cite{Modiano,modiano_age,age_power,gunduz_aoi_arq,Age_engy_fading,Age_power_lyapunov,update_wait}. AoI minimization in multi-user  cases with users communicating over wireless on-off   \cite{Modiano,modiano_age} and fading  \cite{age_power, gunduz_aoi_arq} channels have been considered.   In multi-user  cases, the works, \cite{Modiano, age_power, gunduz_aoi_arq, Age_engy_fading,Age_power_lyapunov} consider orthogonal multiple access (OMA) technique, such as  time-division multiple-access (TDMA), and the works, \cite{generate_will_rvb,NOMA_adaptive_MDP,NOMA_downlink_Satellite_PSO,aloha_noma} consider non-orthogonal multiple access (NOMA) scheme. AoI minimization with various constraints, including energy constraints \cite{Age_engy_fading, age_power}, has been studied. For status update packet arrivals, generate-at-will \cite{age_power, gunduz_aoi_arq} and exogenous arrival \cite{modiano_lowerbound}  models have been considered. %have been considered for information sources. 

%The authors in \cite{modiano_age} obtains low-complexity scheduling policies that minimize AoI for multi-user case in a on-off wireless channel setting.
 
In the above works, the status updates are not required to be processed for being useful, and hence, the AoI is a function of the time interval between consecutive update generations and the transmission time. However, in applications where the raw information needs to be processed before it can be used, the freshness of a status update also depends on the time required for data processing \cite{jr_reviewer31}. 
In order to account for this, we use a metric referred to as the  age of processed information (AoPI), where the instantaneous AoPI is  defined as the time elapsed since the generation of latest received processed status update at a destination, similar to \cite{AoPI}. 

In practice, the information  sources are usually constrained by energy and  computational resources, due to which the task of processing the generated data, locally at the sources, may be expensive or prohibitive. In this case, the data processing task may be offloaded to an edge server, as considered in \cite{AoPI,AoT, Single_LC_EC_PC,Single_Only_Edge, mec_lyapunov,mec_fading_lyapunov,dynamic_age_mec_lyapunov,age_edge_res_alloc}. The works, \cite{AoPI,AoT, Single_LC_EC_PC,Single_Only_Edge} consider AoI minimization with edge server for single-user case. AoI minimization with edge server in multi-user scenario has been studied in \cite{mec_lyapunov,mec_fading_lyapunov,dynamic_age_mec_lyapunov,age_edge_res_alloc}.
The authors in \cite{age_edge_res_alloc} consider age minimization with computation offloading under average energy, time, bandwidth and computational resource allocation constraints in an  \emph{orthogonal} multiple access channel setting. They assume  the transmission power of the mobile device to be a constant and communication to the edge server occurs over a fading channel, due to which, the time taken for the transmission of status updates to the edge server varies, based on the channel conditions. 
Unlike in \cite{age_edge_res_alloc}, we consider the case when the source node has channel state information at the transmitter (CSIT). Using CSIT, the source node controls the transmit power to deliver status updates to the edge server over a fixed amount of time.  Moreover, unlike in \cite{age_edge_res_alloc}, we consider a NOMA scheme.  The adoption of the NOMA scheme and the power control mechanism introduce new challenges in the current work, in comparison to earlier works that consider AoPI optimization with edge computing.  

The works \cite{AoPI, mec_lyapunov,mec_fading_lyapunov,dynamic_age_mec_lyapunov,age_edge_res_alloc,Single_Only_Edge,AoT,Single_LC_EC_PC}  consider that the source devices can communicate to the edge server via OMA technique. Unlike in them,  we consider that the sources can communicate to the BS using a NOMA technique.  
The NOMA scheme has been considered for AoI optimization in  a fading MAC, when no processing is involved,  in \cite{generate_will_rvb, jr_reviewer32, NOMA_adaptive_MDP,NOMA_downlink_Satellite_PSO}. %In \cite{generate_will_rvb}, the authors obtained a stationary randomized policy, for deciding which user and with what power the status updates to be transmitted to the BS for AoI minimization. 
%The result of \cite{generate_will_rvb} are not applicable to the current case, because,
%\cite{generate_will_rvb}, when no processing was involved. The results of 
When processing is involved, in a multi-user case, \cite{aloha_noma} considers a slotted-ALOHA based NOMA for offloading  computation tasks to one of the multiple cores available at the edge server, where the users  can  select one of the two possible  transmit powers for offloading. 
Compared to \cite{generate_will_rvb,NOMA_adaptive_MDP,NOMA_downlink_Satellite_PSO}, in the current paper, we need to jointly optimize scheduling the local and edge processing tasks, and compared to \cite{aloha_noma}, we need to optimize transmit powers when communicating over a fading MAC, due to which, our work is significantly different from them. 

In this work, we  consider users equipped with sensors and actuators, where the sensors generate updates that need to be processed for driving the actuators that are collocated at the user itself. This models many practical cyber-physical-system (CPS) users where both sensing and actuation are carried out by the same CPS device \cite{SameDevice}. In this setting, we study the problem of minimizing the average AoPI across all the devices under the average power consumption constraint for each device in a wireless fading channel environment. 
We consider time-slotted system and the generate-at-will model as in \cite{Modiano, generate_will_rvb, generate_will_kadota}, in which packets can be generated at the start of a slot. We adopt the NOMA strategy, where multiple  users can transmit data to the BS simultaneously subject to the achievable rate region of the underlying MAC. At each slot, decision has to be made on which users must sample a data packet and whether their data should be processed locally or at the edge server. The trade-off involved while taking the decision is the following: To generate a status update and locally process it, the power expended can be greater than the power required for  transmission to the edge server. At the same time, as the channel power gain is random and due to the interference among the users, waiting for a good channel realization and low interference among the users, for transmitting (at a low power) and processing the data at the edge server may  increase the AoPI.  However,  transmitting with a high power when the channel is poor may increase the average power consumption.  Hence, there exists a trade-off between choosing to process at the local processor or the edge server, for minimizing AoPI subjected to a constraint on the average power consumption.
Towards this, the main contributions of the  paper are:
\begin{itemize}
	\item We cast the AoPI minimization problem as a Constrained Markov Decision Process (CMDP) and use a Lagrangian relaxation to obtain an unconstrained MDP. We prove that the  optimal actions for the unconstrained MDP have  a threshold structure with respect to age and channel power gains, which can be exploited for efficient computation and implementation of the policy. We also optimize the Lagrange dual variables via primal-dual algorithm \cite{primal_dual}.
	\item We propose a low-complexity Drift-Plus-Penalty (DPP) method based on Lyapunov optimization to solve the optimization problem. Using the lower bound to the original optimization problem, we quantify the performance gap between the solution obtained from drift-plus-penalty method and the optimal solution of the original problem. 
	\item Via numerical simulations, we illustrate the threshold structure of the optimal actions   for the unconstrained MDP with respect to age and channel power gains. We also show the variation of average AoPI obtained from the CMDP and DPP based solutions and other simpler policies, with respect to the upper bound on the average power constraint.   	
	Further, we obtain the largest achievable AoPI region of the DPP policy and the variation of long-term AoPI achieved by the DPP policy  and a greedy policy,  when the number of users in the network is varied.
\end{itemize}
The current work considers a generate-at-will packet arrival model and assumes perfect CSIT. As part of future work, it may be interesting to consider an exogenous packet arrival model and  make no or imperfect CSIT assumptions. % make no or imperfect CSI assumption.} 
The rest of this paper is organized as follows. In Section II, we present the system model and problem formulation, which is solved in Section III. Numerical results are presented in Section IV and the paper is concluded in Section V.

==> Literature_survey.tex <==
\cite{9685691} solves the problem of minimizing average age over dual hop system by optimizing block-lengths for both hop using an approximate decoding error probability given as function of block-length.

\cite{9500826} optimizes expected age for wireless power transmission systems over rounds where each round has energy harvesting, information collection with energy expense and information transmission with energy expense. It tries to minimize expected age via optimizing the rounds time with QoS and energy constraints.

\cite{9145084} studies AoI outage with respect to blocklength allocation problem and develops an algorithm to reduce AoI outage.

\cite{8445909} minimizes average age by finding an optimal blocklength which also reduces serice time of automatic repeat request (ARQ)

\cite{9665727} jointly formulates average age and AoI violation and proves the existance of optimal blocklength to minimize average age.

\cite{9024516} minimizes average network AoI in a wireless sensor network with multiple users optimizing on blocklength allocated to each user.

\cite{9804773} maximizes throughput by optimizing blocklength and power allocated to each user in a network

\cite{8836117} minimizes average age as well as resources at a controller which receives information from multiple sensors by optimizing over blocklength, power and status updates during each slot (imp) 

\cite{8437671} studies delay and peak AoI in a point-to-point communication system and stresses on importance of delay violation probability rather than average delay and finds blocklengths capable of lesser delay violation probability

\cite{9400231} AoI driven statistical delay and error rate bound in finite blocklength regime for a better QoS (less understood)

In our work we minimize long term average AoI in a network by designing a policy over transmitting a set of resources

In the literature, in most of the problems which consider the scheduling of code rate and power allocation, it is either assumed that for any rate and power combination, the channel capacity formula holds and hence no error is incurred or the relationship between block error incurred is captured using the normal approximation bound of PPV. 
In many applications, one often needs to schedule code rates
The main contribution of the work is, when the codewords (whose characteristic gets reflected in terms of codeword lenghts, code rate and block error probability) and schedu
\begin{itemize}
    \item 
\end{itemize}


==> Solution.tex <==
In this section, we first solve \eqref{AoP} via the CMDP framework and obtain several structural properties of the solution. We then propose  a sub-optimal drift-plus-penalty policy based on Lyapunov optimization and obtain a bound on the ratio of the AoPI achieved by the policy and the optimal AoPI, $A^*$ in \eqref{AoP}.  

\subsection{Solution via the Constrained MDP Framework}
For formulating \eqref{AoP} as a CMDP, in the below, we first identify the components of CMDP corresponding to  \eqref{AoP}.
\paragraph{State Space, $\mathcal{M}$}
We consider the state in slot $k$ for user $m$ to be,
$s_m(k) = (a_m(k), h_m(k))$, where $a_m(k)$ is the instantaneous AoPI and $h_m(k)$ is the channel power gain, of user $m$ in slot $k$. 
%The channel power gain of users are independent and identically distributed (i.i.d.) random variables taking a finite set of values.
% 	Need to specify that channel power gain values belong to a finite set (discrete set of values) 
The state vector in slot $k$, $\mathbf{s}(k) \triangleq  (\mathbf{a}(k), \mathbf{h}(k)) $, where, $\mathbf{a}(k) \triangleq (a_1(k),a_2(k),\dots, a_M(k))$ and $ \mathbf{h}(k) \triangleq (h_1(k), h_2(k), \dots, h_M(k)) $. Therefore, the state space, $\mathcal{M} \subseteq \{1,2,\dots\}^M \times \mathcal{H}_1\times \ldots \times \mathcal{H}_M$.

\paragraph{Action Space, $\mathcal{A}$} 
The action in slot $k$ is given as, $(\mathbf{I}_{e}(k), \mathbf{I}_{l}(k), \boldsymbol{\theta}(k))$, where $\mathbf{I}_{e}(k) = (I_{e,1}(k), \dots, I_{e,M}(k))$,  $\mathbf{I}_{l}(k) = (I_{l,1}(k), \dots, I_{l,M}(k))$, $\boldsymbol{\theta}(k)$ denotes the decoding order for users and $I_{e,m}(k), I_{l,m}(k) \in \{0,1\}$. 
Hence, the action space $\mathcal{A} \subseteq \{0,1\}^M \times \{0,1\}^M \times \mathcal{P}$, where $\mathcal{P}$ is the set of all possible decoding orders of the users. 

\paragraph{State Transition Probabilities}
From \eqref{AoP_def} and channel power gain distributions, we can obtain the state transition probability, $P_{\mathbf{s},\mathbf{s}'} \left(\mathbf{I}_{e}(k),\mathbf{I}_{l}(k), \boldsymbol{\theta}(k)\right)$,   for transition from state $\mathbf{s}$ to $\mathbf{s}'$ when action $\left(\mathbf{I}_{e}(k),\mathbf{I}_{l}(k), \boldsymbol{\theta}(k)\right)$ is taken.
\paragraph{Instantaneous Cost}
%The instantaneous cost includes the AoP cost and the energy consumption cost.
The instantaneous costs for state, $\mathbf{s}(k)$ and  action,  $(\mathbf{I}_{e}(k),\mathbf{I}_{l}(k), \boldsymbol{\theta}(k))$ pair are: (i) individual AoPI cost, $a_m(k+1)$ %at user $m \in \{1,2,\dots,M\}$ 
and (ii) individual power consumption, %cost, 
$P_m(k) = P_{e,m}(k)I_{e,m}(k)
+ P_{l,m}I_{l,m}(k)$, $\forall m \in \{1,\dots,M\}$. From \eqref{decoding_order}, note that $P_{e,m}(k)$ depends on the set of users that transmit to the edge server and their decoding order. 

Under the above setting, we define the long-term weighted average expected AoPI and power consumption cost functions for a policy $\pi$ that maps from $\mathcal{M}$ to $\mathcal{A}$ with initial state $\mathbf{s}_0$ as
\begin{align}
	& A^{\pi}(\mathbf{s}_0) = \lim_{K \to \infty} \frac{1}{MK}\mathbb{E}_{\pi}\sum_{m=1}^{M}\sum_{k=1}^{K}\left[w_ma_{{m}}(k)|\mathbf{s}_0\right], \nonumber \\
	& P^{\pi}_m(\mathbf{s}_0) =  \lim_{K\rightarrow \infty} \frac{1}{K}  \mathbb{E}_{\pi} \sum_{k=1}^K\left[P_{m}(k)|\mathbf{s}_0 \right] \nonumber,
\end{align}
for all $m \in \{1,2,\dots, M\}$. Now,  \eqref{AoP} can be restated as
\begin{align}\label{CMDP}
A^*=	\min_{\pi}  & \; A^{\pi}(\mathbf{s}_0) \;\;	\text{subject to} \;\; P^{\pi}_m(\mathbf{s}_0) \leq \bar{P}_m, 
\end{align}
for all $m \in \{1,2,\dots, M\}$. In the below, we propose Lagrangian relaxation method to obtain the solution to \eqref{CMDP}. 
\paragraph{Lagrangian Relaxation of the CMDP} We relax \eqref{CMDP} into an unconstrained MDP.   We define  instantaneous cost as
\begin{flalign}\label{cost}
	& c_{\boldsymbol{\lambda}}\left(\mathbf{s}(k), \mathbf{I}_{e}(k),\mathbf{I}_{l}(k), \boldsymbol{\theta}(k)\right)
	 =\sum_{m=1}^M w_m a_m(k+1) \nonumber \\
	& \quad \qquad \quad + \sum_{m=1}^M \lambda_m \left(P_{e,m}(k)I_{e,m}(k)
	+ P_{l,m}I_{l,m}(k)\right), 
\end{flalign}
where  $\lambda_m \geq 0$ is the parameter that trades-off the cost due to AoPI and the power expended by user $m$, and  $\boldsymbol{\lambda}\triangleq (\lambda_1,\lambda_2,\ldots,\lambda_M)$. 
Define an  expected $\gamma$-discounted total cost with initial state $\mathbf{s}_0$ under a policy $\pi$ as
\begin{align}\label{main_val_fun}
	V_{\boldsymbol{\lambda},\gamma}^{\pi}(\mathbf{s}_0) = \lim_{K \to \infty} \sum_{k=1}^K\gamma^{k-1} \mathbb{E}\left[c_{\boldsymbol{\lambda}}\left(\mathbf{s}(k), \mathbf{I}_{e}(k),\mathbf{I}_{l}(k), \boldsymbol{\theta}(k)\right)|\boldsymbol{s}_0\right],
\end{align}
where  $\gamma \in (0,1)$ is a discount factor. In this work, for solving \eqref{CMDP}, we take the following approach. We first   obtain a stationary optimal policy, $\pi^*$, which solves 
\begin{equation}\label{eq:val}
	V_{\boldsymbol{\lambda}, \gamma}^*(\mathbf{s}_0) = \min_{\pi} V_{\boldsymbol{\lambda},\gamma}^{\pi}(\mathbf{s}_0). 
\end{equation}
Further, along the lines of \cite[Lemma~$6$]{Modiano}, it can be shown that, $\lim_{\gamma \to 1}(1-\gamma)V_{\boldsymbol{\lambda},\gamma}(\mathbf{s}_0) = V_{\boldsymbol{\lambda}}(\mathbf{s}_0) = V_{\boldsymbol{\lambda}}^*$, for any initial state $\boldsymbol{s}_0$. Finally, we optimize  $\boldsymbol{\lambda}$, i.e., we solve $\max_{\boldsymbol{\lambda}}\left(V_{\boldsymbol{\lambda}}^*-\sum_{m=1}^M \lambda_m\bar{P}_m\right)$ %Under certain technical conditions, it can be shown that strong duality holds and $A^*$ can be obtained from the final step    \cite{primal_dual,altman_cmdp}. 
%We optimize $\max_{\boldsymbol{\lambda}}\left(V_{\boldsymbol{\lambda}}^*-\sum_{m=1}^M \lambda_m\bar{P}_m\right)$   
using the Lagrangian primal-dual approach \cite{altman_cmdp, primal_dual}.
 In the below, we obtain structural properties of the optimal policy, $\pi^*$, that solves \eqref{eq:val}. 
 
For any fixed $\boldsymbol{\lambda}$, the minimum expected total $\gamma$-discounted cost $V_{\boldsymbol{\lambda},\gamma}(\boldsymbol{s})$ for initial state $\boldsymbol{s}$ can be written as
\begin{align}\label{val_func}
	V_{\boldsymbol{\lambda},\gamma}(\mathbf{s}) = & \min_{ \mathbf{I}_{e},\mathbf{I}_{l}, \boldsymbol{\theta}}\left( c_{\boldsymbol{\lambda}}(\mathbf{s}, \mathbf{I}_{e},\mathbf{I}_{l}, \boldsymbol{\theta}) + \gamma \mathbb{E}[V_{\boldsymbol{\lambda},\gamma}(\mathbf{s}')|\mathbf{s}, \mathbf{I}_{e},\mathbf{I}_{l}, \boldsymbol{\theta}]\right),
\end{align}
where
$\mathbb{E}[V_{\boldsymbol{\lambda},\gamma}(\mathbf{s}')|\mathbf{s},  \mathbf{I}_{e} ,\mathbf{I}_{l}, \boldsymbol{\theta}] =  \sum_{\mathbf{s}' \in  \mathcal{M}}P_{\mathbf{s},\mathbf{s}'} \left(\mathbf{I}_{e},\mathbf{I}_{l}, \boldsymbol{\theta} \right)V_{\boldsymbol{\lambda},\gamma}(\mathbf{s}'). \nonumber$
Here, $V_{\boldsymbol{\lambda},\gamma}(\mathbf{s})$ can be obtained by value iteration. This involves iteratively solving the following Bellman equation:
\begin{flalign}
	& V_{\boldsymbol{\lambda},\gamma,n+1}(\mathbf{s}) \nonumber \\ 
	&   = \min_{\mathbf{I}_{e},\mathbf{I}_{l}, \boldsymbol{\theta}} \left( c_{\boldsymbol{\lambda}}(\mathbf{s},\mathbf{I}_{e},\mathbf{I}_{l}, \boldsymbol{\theta})+ \gamma \mathbb{E}[V_{\boldsymbol{\lambda},\gamma,n}(\mathbf{s}')|\mathbf{s},\mathbf{I}_{e},\mathbf{I}_{l}, \boldsymbol{\theta}]\right),\;\forall n\geq0,\nonumber
\end{flalign}
where we define, $V_{\boldsymbol{\lambda},\gamma,0}(\mathbf{s})=0$ and 
\begin{comment}
It can be shown that, as $n \rightarrow \infty, V_{\boldsymbol{\lambda},n}\righarrow V_{\boldsymbol{\lambda}} $
\end{comment}                       
\eqref{main_val_fun} can be written as
\begin{equation}\label{val_q_fun}
	V_{\boldsymbol{\lambda},\gamma}(\mathbf{s}) = \min_{\mathbf{I}_{e},\mathbf{I}_{l}, \boldsymbol{\theta}} Q_{\boldsymbol{\lambda},\gamma}(\mathbf{s},\mathbf{I}_{e},\mathbf{I}_{l}, \boldsymbol{\theta}),
\end{equation}
where, $Q_{\boldsymbol{\lambda},\gamma}(\mathbf{s},\mathbf{I}_{e},\mathbf{I}_{l}, \boldsymbol{\theta}) = c_{\boldsymbol{\lambda}}(\mathbf{s},\mathbf{I}_{e},\mathbf{I}_{l}, \boldsymbol{\theta})+\gamma\mathbb{E}\left[V_{\boldsymbol{\lambda},\gamma}(\mathbf{s}'|\mathbf{s},\mathbf{I}_{e},\mathbf{I}_{l}, \boldsymbol{\theta})\right]. \nonumber $
We have the following result where we obtain the optimal decoding order for given   $\boldsymbol{\lambda}$, $\mathbf{h}(k)$ and optimal $\mathbf{I}_e(k)$ in slot $k$. 
\begin{lemma}\label{decoding order}
 In slot $k$, the optimal decoding order $\theta^*(k)$ of the users for the optimal policy $\pi^*$ satisfies 
\begin{align} \label{eq:decoding-order}
		\frac{\lambda_{\theta^*_1}}{h_{\theta^*_1}} \leq \frac{\lambda_{\theta^*_2}}{h_{\theta^*_2}} \leq \dots \frac{\lambda_{\theta^*_{|\mathcal{T}|}}}{h_{\theta^*_{|\mathcal{T}|}}},
	\end{align}
	where $\theta^*_m \in \mathcal{T}$ is the index of $m^{\rm th}$ user being decoded and $\mathcal{T} \triangleq \{m\; |\; I_{e,m}(k)=1\}\subseteq\{1,2,\dots,M\}$.
\end{lemma}
\begin{proof}
	The optimal decoding order  $\boldsymbol{\theta}^*(k)$ should be selected such that for any given $\mathbf{I}_{e}(k)$ and $\mathbf{I}_{l}(k)$, $Q_{\boldsymbol{\lambda},\gamma}(\mathbf{s}(k),\mathbf{I}_{e}(k),\mathbf{I}_{l}(k), \boldsymbol{\theta}(k))$ is minimized. From \eqref{AoP_def}, we have,  $a_m(k+1)= a_m(k)(1-I_{e,m}(k)-I_{l,m}(k) + I_{e,m}(k)I_{l,m}(k))+1$. Hence, the decoding order $\boldsymbol{\theta}(k)$ for state $\mathbf{s}(k)$  does not influence the next state $\mathbf{s}(k+1)$. Therefore, for any  $\mathbf{I}_{e}(k)$ and $\mathbf{I}_l(k)$, the optimal decoding order $\boldsymbol{\theta}^*(k)$ is selected such that the instantaneous cost is minimized. However, the instantaneous AoPI in the next slot and the power required to locally process the data packet is independent of the decoding order. Hence, from \eqref{cost}, the optimal decoding order  $\boldsymbol{\theta}^*(k)$ in slot $k$ is, 
	\begin{align}\label{eq:opt_order}
		\boldsymbol{\theta}^*(k) = \argmin_{\boldsymbol{\theta} \in \mathcal{P}} \sum _{m=1} ^M \lambda_mP_{e,m}(k)I_{e,m}(k),
	\end{align}
where $\mathcal{P}$ is the set of all possible decoding orders of the users. The problem in \eqref{eq:opt_order} is similar to the optimization problem (57) of \cite{noma_decoding} and the result follows from  (58) and (59) of \cite{noma_decoding}. 
\end{proof}

Due to  Lemma~\ref{decoding order}, the optimal decoding order in \eqref{eq:decoding-order} can be obtained by sorting  $\lambda_m/h_{m}$ for $m\in \mathcal{T}$, which has a polynomial complexity in the number of users. This complexity is significantly lower than  that of searching over  all the possible decoding orders of the users, which exponentially increases with the number of users. In the below theorem, we obtain further results on the structural properties of the optimal solution.  %From \eqref{AoP_def}, we have,  $a_m(k+1)= a_m(k)(1-(I_{e,m}(k)+I_{l,m}(k)) - (I_{e,m}(k)I_{l,m}(k)))+1$. Hence, the optimal decoding order $\theta^*(k)$ for state $\mathbf{s}(k)$  does not influence to the next state $\mathbf{s}(k+1)$. 
Let $\mathbf{x}_{-m} =  (x_1, x_2,\ldots, x_{m-1}, x_{m+1}, \dots, x_M)$.  
%We have the following result: 
\begin{theorem}\label{threshold_struct}
	The following results hold:
  \begin{itemize}
    \item When $\mathbf{a}_{-m},
	\mathbf{h}$ and $\mathbf{I}_{e,-m}$, $\mathbf{I}_{l}$ are fixed and for any arbitrary decoding order $\boldsymbol{\theta}$, the optimal action $I_{e,m}$ is non-decreasing in AoPI, $a_m$. Similarly, when $\mathbf{a}, \mathbf{h}_{-m}$ and $\mathbf{I}_{e,-m}$, $\mathbf{I}_{l}$ are fixed and for any arbitrary decoding order $\boldsymbol{\theta}$, the optimal action $I_{e,m}$ is non-decreasing in   $h_m$.
	\item 	When $\mathbf{a}_{-m},
	\mathbf{h}$ and $\mathbf{I}_{e}$, $\mathbf{I}_{l,-m}$ are fixed and for any arbitrary decoding order $\boldsymbol{\theta}$, the optimal action $I_{l,m}$ is non-decreasing in AoPI, $a_m$. Similarly, when $\mathbf{a},
	\mathbf{h}_{-m}$ and $\mathbf{I}_{e}$, $\mathbf{I}_{l,-m}$ are fixed and for any arbitrary decoding order $\boldsymbol{\theta}$, the optimal action $I_{l,m}$ is non-decreasing in $h_m$.
\end{itemize}
\end{theorem}
\begin{proof} 
	We first show that when  $\mathbf{a}_{-m}$ and $\mathbf{h}$ are fixed, $V_{\boldsymbol{\lambda},\gamma}(a_m,\mathbf{a}_{-m}, \mathbf{h})$ is a non-decreasing function of $a_m$. Then, we prove the first part of the result by showing   $Q_{\boldsymbol{\lambda},\gamma}(a_m, I_{e,m}, I_{l,m},\boldsymbol{\theta},\cdot)$ is sub-modular in $(a_m,I_{e,m})$, when $\mathbf{a}_{-m}, \mathbf{h}, \mathbf{I}_{e,-m}, \mathbf{I}_{l}$ are fixed and $Q_{\boldsymbol{\lambda},\gamma}( h_m, I_{e,m}, I_{l,m},\boldsymbol{\theta},\cdot)$ is sub-modular in $(h_m,I_{e,m})$, when $\mathbf{a}, \mathbf{h}_{-m}, \mathbf{I}_{e,-m}, \mathbf{I}_{l}$ are fixed. Similarly, we prove the second part   by showing   $Q_{\boldsymbol{\lambda},\gamma}(a_m, I_{l,m}, I_{e,m},\boldsymbol{\theta},\cdot)$ is sub-modular in $(a_m,I_{l,m})$, when $\mathbf{a}_{-m}, \mathbf{h}, \mathbf{I}_{e}, \mathbf{I}_{l,-m} $ are fixed and $Q_{\boldsymbol{\lambda},\gamma}(h_m, I_{l,m}, I_{e,m},\boldsymbol{\theta},\cdot)$ is sub-modular in $(h_m,I_{l,m})$, when $\mathbf{a}, \mathbf{h}_{-m}, \mathbf{I}_{e}, \mathbf{I}_{l,-m}$ are fixed. 	See Appendix \ref{Thm:2-proof} for details. 
\end{proof}
%From Theorem~\ref{threshold_struct} we can infer that, the optimal actions $I_{e,m}, I{l,m}$ are monotonic in state variables, $a_m$ and $h_m$ when all other state and action variables are fixed except the state variable and action variable pair.  
Due to Theorem~\ref{threshold_struct}, calculation of state-action value function, $Q_{\boldsymbol{\lambda},\gamma}(\cdot,\cdot)$ for every state-action pair is not necessary, since the optimal actions for some states can be obtained by comparing the corresponding state variable values  with the thresholds whose optimal actions are already known. 
This reduces computational complexity of   value iteration algorithm, as in  \cite{Modiano}.
The complexity of the CMDP based approach even after exploiting Theroem~\ref{threshold_struct} may prohibit computation of the optimal policy when  the number of state and actions are large. For such cases, in the below, we obtain simpler policies. 

\subsection{Drift-Plus-Penalty (DPP) Method} 
We adopt the DPP method based on Lyapunov optimization for obtaining a simpler but sub-optimal policy for solving \eqref{AoP}. We also bound its performance. 
%We begin by defining a virtual queue, Lyapunov function and Lyapunov drift. 
Define a virtual queue $\mathbf{Q}(k) = \{Q_1(k), Q_2(k), \ldots, Q_M(k)\}$, where
\begin{flalign}\label{eq:queue}
	& Q_m(k+1) = \max\{Q_m(k)-\bar{P}_m, 0\} \nonumber \\
	& \qquad \qquad \qquad + P_{e,m}(k)I_{e,m}(k)+P_{l,m}(k)I_{l,m}(k),
\end{flalign} 
for $m \in \{1,2,\dots,M\}$ and $k \in \{1, 2,\dots\}$. The transmit power of user $m$, $P_{e,m}(k)$ for a given decoding order $\boldsymbol{\theta}(k)$ can be computed using \eqref{decoding_order}. 
Let $S(k)= \{Q_m(k)\}_{m=1}^M$ be the state of the system at time slot $k$. %where $P_m(k) = P_{e,m}(k)I_{e,m}(k)+P_{l,m}(k)I_{l,m}(k)$.   
The conditional Lyapunov drift that measures the expected change of Lyapunov function over slots given the state of the system $S(k)$ in slot $k$ is 
\begin{align} \label{sk}
	\Delta(S(k))   = \mathbb{E}[L(Q(k+1))  - L(Q(k))| S(k)],  
\end{align}
where  $L(Q(k))$ is  defined as $	L(Q(k)) = \frac{1}{2}\sum_{m=1}^{M} Q^2_m(k)$. 
In  DPP method, a solution to \eqref{AoP} is obtained by solving  \cite{Neely}: 
\begin{subequations} \label{DPP}
	\begin{align}
		\text{minimize} \;\;&  \Delta(S(k)) + \beta\sum_{m=1}^{M}\mathbb{E}[w_ma_m(k+1)|S(k)],\label{eq:DPP_obj} \\
		\text{subject to} \;\; 
		& I_{e,m}(k), I_{l,m}(k)\in \{0,1\},  
	\end{align}
\end{subequations}
where $m \in \{1,2,\dots, M\}$ and $k \in {\{1,2,\dots\}}$. Here, $\beta > 0$ is the parameter that trades-off the importance of the penalty function i.e., the sum-average AoPI of all the users and the Lyapunov drift $\Delta(S(k))$ and $w_m > 0$ is the weight assigned to the user $m$. Instead of solving \eqref{DPP}, as in \cite{Neely}, we obtain an upper bound to \eqref{eq:DPP_obj} and show that the AoPI obtained by minimizing the upper bound is  %such an algorithm can achieve the AoPI which 
is arbitrarily close to $A^*$ in \eqref{AoP}.  
It can be shown that
%The conditional Lyapunov drift, $\Delta(S(k))$ can be upper bounded as given below: %(see \cite{longerversion}):
%\begin{flalign} \label{upper_bound}
	$\Delta(S(k)) \leq M B + \sum_{m=1}^{M} Q_m(k) (\mathbb{E}\left[P_m(k)|S(k)\right]- \bar{P}_m),$
%\end{flalign}
where $B \geq \frac{1}{2M}\sum_{m=1}^{M}(\bar{P}_m^2+ \mathbb{E}\left[{P_m^2(k)}|S(k) \right])$.
Let $B = \frac{1}{2 M}\sum_{m=1}^{M} (\bar{P}_m^2 +  (\max_{\boldsymbol{\theta},\mathbf{h}} \{P_{e,m}(h_m)\}_{m= 1}^{M}+P_{l,m})^2)$. Here, $ \max_{\boldsymbol{\theta},\mathbf{h}} \{P_{e,m}(h_m)\}_{m= 1}^{M}$ is obtained assuming $I_{e,m}=1, \; \forall m \in \{1,\dots,M\}$. 
%and $\theta \in \mathcal{P}_M$, where $\mathcal{P}_M$ is the set of all possible decoding orders when all $M$ users have $I_{e,m}=1$ and $\mathbf{h} \in \mathcal{H}_1\times \ldots \times \mathcal{H}_M$ .
 Hence, $B$ does not depend on the actions, $\mathbf{I}_{e}(k), \mathbf{I}_{l}(k)$ and the decoding order, $\boldsymbol{\theta}(k)$ in slot $k$.  
Using the above upper bound on $\Delta(S(k))$, we obtain: 
\begin{subequations}\label{eq:DPP_greedy} 
	\begin{align}
\mini_{\mathbf{I}_e, \mathbf{I}_l,\boldsymbol{\theta}} \label{eq:DPP_objective}\;& \frac{1}{2}\sum_{m=1}^{M} \left(Q_m(k) (P_m(k)- \bar{P}_m) +\beta w_m a_m(k+1) \right), \\
\text{subject to} \;\; 
		& I_{e,m}(k),I_{l,m}(k)\in\{0,1\},  
	\end{align}
\end{subequations}
where $a_m(k+1)= a_m(k)(1-I_{e,m}(k)-I_{l,m}(k) + I_{e,m}(k)I_{l,m}(k))+1$, $P_m(k) = P_{e,m}(k)I_{e,m}(k)+ P_{l,m}I_{l,m}(k)$, $\forall m \in \{1,2,\dots,M\}$ and $P_{e,m}(k)$ depends on the decoding order $\boldsymbol{\theta}_m(k)$.
We refer to the policy obtained by solving \eqref{eq:DPP_greedy} as the DPP policy   and denote the optimal long-term weighted average AoPI achieved by the DPP policy by $A_{\rm DPP}$. 

The problem in \eqref{eq:DPP_greedy} is solved as follows. At each $k$, the network state, $\mathbf{Q}(k)$ and the channel state, $\mathbf{h}(k)$ are observed and the action $(\mathbf{I}_{e}(k), \mathbf{I}_{l}(k),\boldsymbol{\theta}(k))$ is taken to minimize the objective \eqref{eq:DPP_greedy} in a greedy manner and the virtual queues are updated according to \eqref{eq:queue}.   
Along the lines in Lemma~\ref{decoding order}, for any given $\mathbf{I}_{e}(k)$ and $\mathbf{I}_{l}(k)$, it can be shown that the optimal decoding order $\boldsymbol{\theta}^*(k)$ for all $m \in \mathcal{T}$ is given by: % $\boldsymbol{\theta}$ that satisfies
%\begin{equation}
%h_{\theta^*_1}(k) \geq h_{\theta^*_2}(k) \geq \dots h_{\theta^*_{|\mathcal{T}|}}(k).
%\end{equation}
\begin{align} \label{eq:decoding-order1}
	\frac{Q_{\theta^*_1}(k)}{h_{\theta^*_1}(k)} \leq \frac{Q_{\theta^*_2}(k)}{h_{\theta^*_2}(k)} \leq \dots \leq \frac{Q_{\theta^*_{|\mathcal{T}|}}(k)}{h_{\theta^*_{|\mathcal{T}|}}(k)},
\end{align}
where $\theta^*_m \in \mathcal{T}$ is the index of $m^{\rm th}$ user being decoded and $\mathcal{T} \triangleq \{m\; |\; I_{e,m}(k)=1\}\subseteq\{1,2,\dots,M\}$.



In \eqref{eq:DPP_greedy},  we do not consider the expectation operator as we opportunistically minimize the objective function for each realization of the channel power gain, leading to minimization of the expected value \cite{Neely}. We summarize the DPP based policy in Algorithm~\ref{algo:DPP}.
\begin{algorithm}[t] 
	\caption{DPP Algorithm}
	 \label{algo:DPP}
	\begin{algorithmic}[1]
		\STATE \textbf{Initialization:} $k =1$, $Q_m(1) = 0$ and sample $\mathbf{h}(1){\raise.17ex\hbox{$\scriptstyle\sim$}} \mathbb{P}(\mathbf{h})$.
		\STATE \textbf{Input:}  $\bar{P}_m \; \text{and} \; P_{l,m} \;\; \forall m$ and  $K\gg 1$.
		\WHILE {$k \leq K$}
		\STATE For different actions, compute the total power consumed for each user.
		\STATE Choose the action that minimizes \eqref{eq:DPP_objective}.
		%\STATE Solve  \eqref{eq:DPP_greedy}.
	    \STATE Update $Q_m(k+1) \; \forall m$ using \eqref{eq:queue}.
		\STATE Update $k \leftarrow k+1$ and sample $\mathbf{h}(k){\raise.17ex\hbox{$\scriptstyle\sim$}}\mathbb{P}(\mathbf{h})$.
		\ENDWHILE
	\end{algorithmic}
\end{algorithm}
We now  derive a   bound on the AoPI, $A_{\rm DPP}$, obtained by optimally solving  \eqref{eq:DPP_greedy}.   
For this, consider 
\begin{subequations}\label{AoP_LB}
	\begin{align}
	A_L =  \min_{\pi}&\lim_{K \to \infty}\frac{1}{2M}\sum_{m=1}^{M}w_m\left(\frac{1}{\frac{1}{K}\sum_{k=1}^{K} \mathbb{E}\left[u_m(k)\right]}+1\right),\\
	\text{subject to, } &	\lim_{K\rightarrow \infty} \frac{1}{K} \sum_{k=1}^K \mathbb{E}_{\pi}\left[P_{m}(k) \right] \leq{\bar{P}_m},\\
	&\;\; I_{e,m}(k), I_{l,m}\in \{0,1\}, 
	\end{align}
\end{subequations}
where $k \in \{1,2,\dots\}$, $m=\{1,2,\dots,M\}$ and   $u_m(k)=1$, if user $m$ receives a processed packet successfully in slot $k$ either from local  or edge processor, else $u_m(k)=0$. It can be shown that $A_L\leq A^*$ based on \cite{modiano_lowerbound}. We now have the following theorem, which is motivated by a result in \cite{modiano_lowerbound}. 
\begin{theorem}\label{opt_ratio}
The following holds:  
	\begin{equation}
	\frac{A_{\rm DPP}}{A^*} \leq 2 + \frac{1}{A_L}\left(\frac{B}{\beta} - 1\right),
	\end{equation}
where $A_L$ is obtained from \eqref{AoP_LB}. When $ \beta = B $, $A_{\rm DPP}\leq 2A^*$. 
\end{theorem}
\begin{proof}
We first show that the virtual queues, $Q_m(k) \; \forall m \in \{1,2,\dots,M\}$ are strongly stable under the DPP policy, which implies that \eqref{averageEnergy} is satisfied \cite[Theorem 2.8]{Neely}.  We then define a class of policies referred to as the channel-only policies,  where the decision is made based on channel power gain vector, $\mathbf{h}(k)$ in slot $k$, for \eqref{eq:DPP_greedy},  and show that the minimum AoPI achieved by them can be arbitrarily close to the optimal solution of \eqref{AoP} \cite{Neely}.   Then, we show that the optimal long-term weighted average AoPI of DPP policy is upper bounded as follows: $A_{\rm DPP}\leq {B}/{\beta} + A^*$. From this and  the lower bound, $A_L$, we complete the proof. See Appendix B for details. 
\end{proof}



\subsection{Relaxed DPP}
We relax $I_{e,m}(k)$, $I_{l,m}(k)$ to take values over $[0,1]$. Under the decoding order in  \eqref{eq:decoding-order1} with $|\mathcal{T}| = M$, $\sum_{m=1}^M Q_m P_m$
is convex. The term $I_{e,m}(k)I_{l,m}(k)$ in \eqref{eq:DPP_greedy} can be dropped  in case the constraint, $I_{e,m}(k)+I_{l,m}(k)\leq 1$, is imposed, and  \eqref{eq:DPP_greedy} can be relaxed to the following convex 
 program:
\begin{subequations}%\label{eq:relaxedDPP}
		\begin{align*}
		\mini_{\mathbf{I}_e, \mathbf{I}_l} \;& \frac{1}{2}\sum_{m=1}^{M} \left(Q_m(k) (P_m(k)- \bar{P}_m) +\beta w_m a_m(k+1)\right), \\
		\text{subject to} \;\; 
		& I_{e,m}(k)+I_{l,m}(k)\leq 1, \\
		& I_{e,m}(k), I_{l,m}\in [0,1],
		\end{align*}
	\end{subequations}
where $a_m(k+1)= a_m(k)(1-I_{e,m}(k)-I_{l,m}(k))+1$ and $P_m(k) = P_{e,m}(k)I_{e,m}(k)+ P_{l,m}I_{l,m}(k)$, $\forall m \in \{1,2,\dots,M\}$. We then solve it using standard numerical techniques and round the obtained ${I}_{e,m}$ and ${I}_{l,m}$ values. %for all $m\in \{1,2,\ldots,M\}$. 

\begin{figure*}[t]
	\centering
	\begin{subfigure}{0.48\textwidth}
		\input{MDP_AoPI_PowerGain_w46}
		\caption{Optimal actions in a $2$-user case for different  $(a_1,h_1)$ when $a_2= 5,  h_2 = 2$.} 
		\label{fig:Threshold_struct_powergain_weights}
	\end{subfigure} 
	\hfill
	\begin{subfigure}{0.48\textwidth}
		\input{MDP_Threshold_Structure_h23_w46}
		\caption{Optimal actions in a $2$-user case for different   $(a_1,a_2)$ when $h_1= 2, h_2 = 4$.}
		\label{fig:Threshold_struct_weights}
	\end{subfigure}	
	\caption{Optimal actions in a two-user case when parameters,  $w_1 = 0.4, w_2 = 0.6, \lambda_1 = 15, \lambda_2 = 20$, $P_{l,1}= 2$ and $P_{l,2}= 3$. 
		In Fig. \ref{fig:Threshold_struct_weights}, $I_{l,1}=I_{l,2}=0$ for all $(a_1,a_2, h_1=2,h_2=4)$ 
		and when $I_{e,1}=I_{e,2}=1$, the optimal decoding order is $\theta_1=2, \theta_2=1$.}
	\label{fig:Optimal Actions}
\end{figure*}

\begin{figure*}[t]
	\centering
	\begin{subfigure}{0.49\textwidth}
		%\centering
		\resizebox{0.99\textwidth}{!}{%
			\input{AoPI_Pbar_JR}
			\phantomsubcaption
			\label{fig:AoPI_Pbar}
		}

	\end{subfigure} 
	\hfill
	\begin{subfigure}{0.49\textwidth}
		\resizebox{0.99\textwidth}{!}{%
			\input{DPP_Age_Pbar_Diff_V}
			\phantomsubcaption
			\label{fig:AoPI_Pbar_beta}
		}

		
	\end{subfigure}	
	\caption{Variation of the average AoPI with the bound on the average power consumption, $\bar{P}$ for a two-user case with  $\bar{P}_1=\bar{P}_2 = \bar{P}$,  under CMDP-based Policy, Drift-Plus-Penalty (DPP) Policy, Relaxed Drif-Plus-Penalty (DPP) Policy with $\beta=4$, Local-Edge, Edge-Only and Local-Only Greedy Policies, and Randomized Fixed-Power Policy in Fig. \ref{fig:AoPI_Pbar} and under the Drift-Plus-Penalty (DPP) Policy for different $\beta$ values in Fig. \ref{fig:AoPI_Pbar_beta} when $P_{l,1}=P_{l,2}=2$. For Randomized Fixed-Power Policy, the probability of selecting edge server to process the data was chosen to be $0.3$ with fixed power required to transmit the data to the edge server being equal to $1.5$ units.}
	\label{fig:AoPI_Pbar_fig}
\end{figure*}

\subsection{Greedy Policies}
We now propose   low-complexity  policies called Local-Edge Greedy, Edge-Only Greedy and Local-Only Greedy policies. 
%that do not take the instantaneous AoPI into account while making the decision in a slot. 
\subsubsection{Local-Edge Greedy Policy}
In this policy, a user samples and processes a packet locally in a slot, if its local processing power is less than the transmit power required for delivering packets successfully to the edge server and if the average power consumed until the slot is less than its bound assuming local processing. Among the remaining users, we find the set of all users which when deliver packets successfully, the  resulting average power consumed until the slot is less than their bound,  assuming no interference among the users. The users outside the set do not sample packets in the slot. The users in the set are assumed to be decoded in the decreasing order of their channel power gains. The transmit powers required are computed starting from the user with the lowest channel power gain. In the process, if a user's transmit power is such that the resulting average power is greater than its bound, we drop the user from the set and continue the process. The users present at the end of the process will transmit in the slot. 
\subsubsection{Edge-Only Greedy Policy}
In this policy, we consider that only the edge processor is available for processing. The users which transmit in a slot and their transmit powers are computed exactly as carried out for the users that do not process locally in the Local-Edge Greedy Policy. 
\subsubsection{Local-Only Greedy Policy}
In this policy, only the local processor is present,  and a user samples and processes a packet locally in a slot, if its local processing power is such that the average power consumed until the slot is less than its bound.
\subsection{Randomized Fixed-Power Policy}
In this policy, %the BS is assumed to not have CSI of the users. 
at the start of a slot, a user randomly proposes for local or edge processing a packet with a certain probability. If the proposal is to process locally, it is accepted if the resulting average power is less than or equal to its bound. Otherwise, the proposal is rejected.  If the proposal is to process at the edge server and the fixed power selected is less than the power required to successfully deliver a packet, assuming no interference among the users, the user transmits with the fixed power. The BS decodes the users according to their decreasing order of the channel power gain. The decision to process the packet at each user is made without CSI. The transmission (and hence the edge processing) will be successful if the transmit power was greater than or equal to the actual transmit power calculated according to the decoding order. 



==> System_model.tex <==


 We consider a multiple access communication system where $M$ users communicate status update packets to a common base station using time-division multiple access. 
The system is time-slotted with unit-length slots which are indexed by $t\in \{1,2,\ldots\}$, where in a slot a single user can transmit a maximum of $N$ symbols. 
At the start of slot $t$, a $k$-bit status update packet, $m_t$, can be generated at will. The transmitter appends $c$-bit CRC to the message bits, encodes them  using an encoder, $\mathcal{E}_t$, to obtain an $n$-symbol channel packet, $x_t =\mathcal{E}_t(m_t,P_t,n)$, where $n\leq N$ for some positive integer $N$. 
The CRC selected is assumed to have 

%Note that we allow the operation performed at the transmitter to vary over time. 
At slot $t$, let $P \in \mathcal{P}$ be the power allocated to a channel packet for transmission, i.e., $||x_t||^2_2=P$.
%In this case, the state of the battery evolves as follows: 
%\begin{align}
%\label{eq:battery evolution}
%    B_{t} = \max(\min(B_{t-1}+E_t,B_{\rm max}) - P_t,0),\; \text{for}\; t %= 1,2,\ldots,
%\end{align}
%where $B_0$ is the initial amount of energy stored in the battery. 
The obtained packet,  $x_t$ is transmitted over the air channels.   
%At any slot $t$, $B_{t}=0$ results in termination of transmission.
The receiver receives the symbols,  $y_t = h(x_t) + w_t$, where $w_t$ is the additive noise random variable of variance and $h(\cdot)$ is the channel that models all the blocks from the modulator to until I/Q samples are received at the receiver. 
The receiver performs operation $\mathcal{D}_t$ to obtain an estimate of the transmitted CRC-appended message sequence on which CRC check is performed, which may fail or pass. 
%$\hat{m}_t$ of the transmitted status update, $m_t$, i.e., $\hat{m}_t=\mathcal{D}_t(y_t)$.
%Under encoder, $\mathcal{E}_t$ and decoder, $\mathcal{D}_t$, let $\epsilon(P_t,n_t)$ be the probability of packet (block) error rate. In emerging ultra-reliable low-latency communication (URLLC) systems, it is important to receive packets of low error (high reliability) \cite{CRC-Assisted-SC}  with low latency or high freshness. 
As discussed, in this work, we are interested in communicating the information as freshly as possible. For this, we use the following metric for every user $i$: 
\begin{align}\label{eq:age_evolution}
\Delta_{t+1}(i) = \begin{cases}
%\Delta_t + N &\text{if $\epsilon(P_t,n_t)\geq \epsilon_{\rm th}$},\\
\Delta_{t}(i) + N  & \text{if $ u_{t,i}=1/0$ and the CRC check fails},\\
n &\text{otherwise},
\end{cases}
\end{align}
which we refer to as the instantaneous age of information (AoI) at time $t$, where $u_{t,i}$ is the indicator variable which takes value $1$ if an information packet is generated in slot $t$ and zero otherwise. When the CRC check fails, we discard the packet and when it passes, we consider the packet as a correct packet, although with a small probability (which decreases with increasing CRC length, $c$) the CRC may pass, but the packet may still be in error.  
Note that the lower the AoI the fresher is the information. 
%where we assume that the time required for decoding is negligible and as soon as $n_t$ noisy symbols are receiver, the $\hat{m}_t$ is available. 
%and $\epsilon_{\rm th}$ is the maximum tolerable packet error. 
Hence, for freshly delivering information, we need to minimize the AoI. For this, we consider the following long-term average AoI minimization problem: 
 \begin{align}\label{eq:main_opt_problem}
P^* = \min_{\pi \in \Pi}& \lim_{T\rightarrow \infty}\frac{1}{TM} \mathbb{E} \left[ \sum_{i=1}^M \sum_{t=1}^T  \Delta_t(i) \right], \\
% \text{subject to}\ & k_i \in \{1, 2, \ldots, n\}\ \forall i,\label{eq:main_policy_constraint}\\
\text{subject to}\ & \sum_{i=1}^{M} u_{t,i}(k,P) \leq 1, \forall t, k, P,  \label{eq:main_policy_constraint}\\
 & \lim_{T\rightarrow \infty}\frac{1}{T}\sum_{t=1}^T  \mathbb{E}[P_i]\leq \bar{P_{\rm max}^i} \ \forall i, \\
 % & 0\leq P_i \leq P_{\rm max}^i,
 & P_i \in \mathcal{P}
 \label{eq:main_pt_constraint}
  \end{align}
for all $t \in \{1,2,\ldots \}$, where the expectation in the objective function is with respect to the randomness in the channel and choice of policy $\pi \in \Pi$. We define our policy for choosing $u_{t,i}(k,P)$ where 
\[u_{t,i}(k,P) = \begin{cases}
1 & \text{if i transmits packet of k-bits with power P},\\
0 &\text{otherwise},
\end{cases}\]
% For each choice of $k_i$ and $P_i$, we choose encoder and decoder pair, $(\mathcal{E}_t^i, \mathcal{D}_t^i)$ $\forall i$, for encoding and decoding the data.
In the current work, we assume that there is a perfect feedback channel that informs regarding whether the CRC passed or failed for a given packet. Using this knowledge, the transmitter maintains instantaneous AoI at the receiver at each slot. 

\section{Solution}
\subsection{Stationary Randomized Policy}
In this subsection, we obtain a stationary randomized policy that has the bounded performance from the optimal solution. The SRP is obtained as a solution to an optimization problem, which we solve via blackbox optimization. 

Let $\mu_i(k,P)$ be the probability with which $k$ bits are encoded to $n$ symbols and transmitted with power $P$ at each slot $t$ at user$-i$. Let $\overline{\epsilon}(k,P)$ be probability of successful reception of symbol  and $U(m)$ be the inter-delivery time for $m^{th}$ packet. 

Consider a policy $\pi$ with scheduling probability matrix $\mu_i(k,P)$ where $k \in \mathcal{K}$ and $P \in \mathcal{P}$. The probability that a certain transmission parameterized by $k,P$ is successful is $\overline{\epsilon_i}(k,P) \mu_i(k,P)$ and the inter-delivery times $U(m)$ is an i.i.d. with a geometric distribution. As AoI renews to $n$ periodically, long term average AoI can be considered as a renewal process  and expressed as

\[\lim_{T\rightarrow \infty}\frac{1}{T}\sum_{t=1}^T  \mathbb{E}[\Delta_t] = \frac{N \mathbb{E}[U^2(m)]}{2 \mathbb{E}[U(m)]}-\left(\frac{N-n}{2}\right)\]
\[=\frac{1}{\overline{\epsilon_i}(k,P) \mu_i(k,P)}\]

% The success probability $p$ can be expressed using block error rate (BLER) as $p = 1- $BLER$(k,P)$. The upper bound on BLER is given in \cite{polyansky}.
% Using the results from \cite{eytan_modiano} and \cite{polyansky}, the optimization problem in \eqref{eq:main_opt_problem} can be reformulated as follows
Where $\overline{\epsilon}(k,P)$ is considered as block error rate which can be upper-bounded using \cite{polyansky}. Using this equation in \eqref{eq:main_opt_problem} gives

\begin{align*}
R^*=\min_{\pi \in \Pi_R} \frac{1}{M} \ & \sum_{i=1}^M \sum_{\mathcal{K},\mathcal{P}} \frac{1}{\overline{\epsilon}_i(k,P) \mu_i(k,P)},  \numberthis \label{eq:modified_opt_problem}\\
\text{subject to}\ & \sum_{i=1}^M \sum_{\{\mathcal{K},\mathcal{P}\}}\mu_i(k,P) = 1 \ ; 0 \leq \mu_i(k,P) \leq 1, \numberthis \label{eq:modified_constraint} \\
 & \sum_{\mathcal{P}} P \sum_{\mathcal{K}} \mu_i(k,P) \leq P_{max}^i, \  \forall i,k,P, \numberthis \label{eq:modified_power_constraint} 
 \end{align*}

 { \color{red}
\begin{align*}
R^*=\min_{\pi \in \Pi_R} & \sum_{i=1}^M\sum_{\mathcal{P}} P \sum_{\mathcal{K}} \mu_i(k,P)  \numberthis \label{eq:modified_opt_problem}\\
\text{subject to}\ & \sum_{i=1}^M \sum_{\{\mathcal{K},\mathcal{P}\}}\mu_i(k,P) = 1 \ ; 0 \leq \mu_i(k,P) \leq 1, \numberthis \label{eq:modified_constraint} \\
& {\sum_{\mathcal{K},\mathcal{P}}\overline{\epsilon}_i(k,P) \mu_i(k,P)}\geq \bar{a}_i
 \end{align*}
  }

\subsection{Performance Bound}
Using \cite{eytan_modiano}, a lower-bound on \eqref{eq:main_opt_problem} can be given as

 \begin{align}\label{eq:lower_bound_opt_problem}
L_B = \min_{\mu_i} \ & \left\{\frac{1}{2M} \left(\sum_{i=1}^{M} \sum_{k,P} \left(2n+ \frac{N}{\bar{\epsilon_i(k,P)\mu_i(k,P)}}-N\right)\right)\right\}, \\
\text{subject to}\ & \eqref{eq:main_policy_constraint}, \eqref{eq:modified_constraint} \ \text{and} \  \eqref{eq:modified_power_constraint}
% \text{subject to}\ & n_t \in \{k, k+1, \ldots, N\},\\
%  & \lim_{T\rightarrow \infty}\frac{1}{T}\sum_{t=1}^T  \mathbb{E}[P_t]\leq \bar{P}, \\
%   & 0\leq P_t \leq P_{\rm max},
  \end{align}
\begin{theorem}
 The optimal value $P^*$ of problem in \eqref{eq:main_opt_problem} is at most twice of $R^*$ that solves \eqref{eq:modified_opt_problem} i.e., $R^* \leq 2P^*$
\end{theorem}
\begin{proof}
 We adopt technique used in \cite{eytan_modiano} to prove our claim. First we obtain a lower-bound on \eqref{eq:main_opt_problem} which is given in \eqref{eq:lower_bound_opt_problem} whose optimal objective $L_B$ is a lower-bound to $P^*$. We then show that the optimal solution to lower-bound problem is also a feasible solution to \eqref{eq:modified_opt_problem}. We then relate objective functions of lower-bound problem, \eqref{eq:modified_opt_problem} and show that $R^* \leq 2P^*$.
%  We then consider an SRP $r \in \Pi_r$ that gives same throughput $q_i^r$ as lower bound throughput $q_i^L$.\\
% $L_B$ in \eqref{eq:lower_bound_opt_problem} can be rewritten as
% \[L_B = \min_{\pi} \ & \left\{\frac{1}{2M} \left(\sum_{i=1}^{M} \sum_{k,P} 2n+ \frac{N}{\bar{\epsilon}_i(k,P,h) \mu_i(k,P,h)}-N\right)\right\}\]

% We define a set $\Lambda_T(h) = \{t : h(t) = h\}$ 
% \[\mu_i^{L}(k,P,h) = \frac{1}{|\Lambda_T(h)|}\sum_{t\in\Lambda_T(h)} E[u_i^{L}(t,k,P)]\]
To verify that solution to the lower-bound is feasible with \eqref{eq:modified_opt_problem}. Consider $\mu_i^*(k,P)$ be an optimal value that solves \eqref{eq:lower_bound_opt_problem}. We can then write
\[\mu_i^*(k,P) = \lim_{T\rightarrow \infty}\frac{1}{T} \sum_{t=1}^T \mathbb{E}[u_{t,i}(k,P)] \ \forall i,k,P\]
where $u_{t,i}(k,P)$ is an indicator variable for $i^{th}$ user transmitting $k$ bits with power $P$. Where $\mu_i^*(k,P) \in \Pi_R$ where $\Pi_R$ is a class of SRPs.
Using $\mu_i^*(k,P)$ in \eqref{eq:modified_opt_problem} gives $R$ and a relation between $L_B$ and $R$ can be given as 
\[L_B = \frac{NR}{2} + \frac{(2n-N)}{2}\]
Using this we can say 
\[\frac{R}{2} < L_B, \  \text{if} \  (2n-N) \geq 0 \]
Note that as $L_B \leq P^* \leq R^* \leq R$. We can give optimality ratio $\psi$ as 
% With $u_i^L(t,k,P)$ as the optimal value that solves $L_B$. It can be proved that constraints \eqref{eq:lb_constraint}, \eqref{lb_constraint2} are satisfied.
% Comparing equations for lower-bound and \eqref{eq:main_opt_problem}, optimality ratio can be given as 
 \[\psi = \frac{R^*}{P^*}\leq \frac{R}{L_B}<2\]


\end{proof}


